Second order accurate distributed eigenvector computation for extremely large matrices

We propose a second-order accurate method to estimate the eigenvectors of extremely large matrices thereby addressing a problem of relevance to statisticians working in the analysis of very large datasets. More specifically, we show that averaging eigenvectors of randomly subsampled matrices efficiently approximates the true eigenvectors of the original matrix under certain conditions on the incoherence of the spectral decomposition. This incoherence assumption is typically milder than those made in matrix completion and allows eigenvectors to be sparse. We discuss applications to spectral methods in dimensionality reduction and information retrieval.

==> FurtherDiscussionExpansionApproxEigen.tex <==
\textbf{INCLUDE A DISCUSSION OF HIGHER-ORDER APPROX}

==> NormCForVerySmallpv1.tex <==
%\subsection{On $\|C\|_2$ when $p$ is extremely small}
At the end of Subsection \ref{ss:sparse-approx}, we mentioned the following fact:
\begin{theorem}\label{thm:LoseControlOfOpNormCForSmallp}
When $p\sim (\log n)^{1-\delta}/n$, and $\delta \in (0,1)$,
$$
\|C/\sqrt{n}\|_2 \tendsto \infty \text{ with probability one. }
$$
\end{theorem}
Let us now justify this claim. (Recall that practically, it suggests that if we don't sample enough the matrix $M$ (i.e $p$ is too small), a subsampling approximation to its eigenproperties is not likely to work.)
\begin{proof}
We consider the case where $p=(\log n)^{1-\delta}/n$, the case $p\sim (\log n)^{1-\delta}/n$ being easily deduced from the special case we consider since $p\sim (\log n)^{1-\delta}/n$ means that we can find $\kappa_1$ and $\kappa_2$ fixed with $n$ such that $\kappa_1 (\log n)^{1-\delta}/n\leq p \leq \kappa_2 (\log n)^{1-\delta}/n$.

Our strategy is to show that the largest diagonal entry of $C\trsp C/n$ goes to infinity. To do so, we will rely on results in random graph theory. Let us examine more closely this diagonal. Using the definition of $C$, we see that, if $T=C\trsp C$, and $d_i$ is the number of times $\sqrt{(1-p)/p}$ appears in the $i$-th column of $C$,
$$
T(i,i)=\frac{np}{1-p}+d_i \left(\frac{1-p}{p}-\frac{p}{1-p}\right)\;.
$$
Now $\{d_i\}$ is the degree sequence of an Erd\"os-Renyi random graph. According to \cite{BollobasRandomGraphs}, Theorem 3.1, if $k$ is such that $n \binom{n-1}{p} p^k (1-p)^{n-1-k}\tendsto \infty$, then, if $X_k$ is the number of vertices with degree greater than $k$,
$$
\lim_{n\tendsto \infty} P(X_k \geq t)=1\;,
$$
for any $t$. So if we can exhibit such a $k$, then $\max d_i \geq k$ with probability going to 1. We now note that for small $p$,
$$
\left(\frac{1-p}{p}-\frac{p}{1-p}\right)\geq \frac{1}{2p}\;.
$$
Hence, if our $k$ is also such that $k/pn\tendsto \infty$, we will indeed have
$$
\max_i \frac{T(i,i)}{n}\tendsto \infty
$$
and the theorem will be proved.\\
We propose to take $k=np+(\log n)^{1-(4\delta)/5}$. According to \cite{BollobasRandomGraphs}, Theorem 1.5, if $h=k-np$, and $q=1-p$,
\begin{equation}\label{eq:KeyEqThmExplosionOpNormC}
\binom{n}{p} p^k (1-p)^{n-k}\geq \frac{1}{\sqrt{2\pi p q n}} \exp\left(-\frac{h^2}{2pqn}-\frac{h^3}{2q^2 n^2}-\frac{h^4}{3p^3n^3}-\frac{h}{pn}-\beta\right)\;,
\end{equation}
where $\beta=1/(12 k)+1/(12(n-k))$. In our case, elementary algebra shows that all the terms in the exponential are negligible compared to $\log n$, hence, as $n\tendsto \infty$,
$$
\sqrt{n}\exp\left(-\frac{h^2}{2pqn}-\frac{h^3}{2q^2 n^2}-\frac{h^4}{3p^3n^3}-\frac{h}{pn}-\beta\right)\tendsto \infty\;.
$$
Therefore, with this choice of $k$,
$$
n \binom{n-1}{p} p^k (1-p)^{n-1-k}\tendsto \infty\;.
$$
So we can finally conclude that
$$
\max_i T(i,i)/n \geq \frac{k}{2np} \text{ with probability going to 1}\;.
$$
But because $(\log n)^{1-(4\delta)/5}\gg np=(\log n)^{1-\delta}$, we have $k/(2np)\tendsto \infty$ and the theorem is proved.
\end{proof}
We note that in the more general case where $p=(\log n)^{1-\delta} u_n/n$, for $0< u_n\leq 1$, the same approach could go through and yield the same result under the following conditions: if we can find $v_n>0$ such that $v_n\tendsto \infty$, while $v_n= o(\log n,[u_n^{-1}(\log n)^{\delta}]^{1/4})$, then by picking $k=np(1+v_n)$ the same proof as above applies. As a matter of fact, under these conditions, it is easy to show that the main term in the exponential appearing in Equation \eqref{eq:KeyEqThmExplosionOpNormC} is $o(\log n)$, which is the key to getting the theorem as we just saw.

